Alleviating Exposure Bias in Diffusion Models through Sampling with Shifted Time Steps

Diffusion Probabilistic Models (DPM) have shown remarkable efficacy in the synthesis of high-quality images. However, their inference process characteristically requires numerous, potentially hundreds, of iterative steps, which could exaggerate the problem of exposure bias due to the training and inference discrepancy. Previous work has attempted to mitigate this issue by perturbing inputs during training, which consequently mandates the retraining of the DPM. In this work, we conduct a systematic study of exposure bias in DPM and, intriguingly, we find that the exposure bias could be alleviated with a novel sampling method that we propose, without retraining the model. We empirically and theoretically show that, during inference, for each backward time step $t$ and corresponding state $\hat{x}_t$, there might exist another time step $t_s$ which exhibits superior coupling with $\hat{x}_t$. Based on this finding, we introduce a sampling method named Time-Shift Sampler. Our framework can be seamlessly integrated to existing sampling algorithms, such as DDPM, DDIM and other high-order solvers, inducing merely minimal additional computations. Experimental results show our method brings significant and consistent improvements in FID scores on different datasets and sampling methods. For example, integrating Time-Shift Sampler to F-PNDM yields a FID=3.88, achieving 44.49\% improvements as compared to F-PNDM, on CIFAR-10 with 10 sampling steps, which is more performant than the vanilla DDIM with 100 sampling steps. Our code is available at https://github.com/Mingxiao-Li/TS-DPM.

==> sec1-introduction.tex <==
\section{Introduction}

Diffusion Probabilistic Models (DPMs) \citep{ddpm,ddpm_ori} are a class of generative models that has shown great potential in generating high-quality images. \citep{NEURIPS2021_beatsgan,ramesh2022hierarchical,Rombach_2022_CVPR, icml22_glide}.
% During training, a given sample $x_0$ is progressively corrupted with Gaussian noise in a series of time steps. The trained DDPM generates synthetic samples by gradually reducing noise level from white noise.
%% xiaoming's version
DPM consists of a forward and a backward process. 
In the forward process, images are progressively corrupted with Gaussian noise in a series of time steps. Conversely, during the backward process, the trained diffusion model generates images by sequentially denoising the white noise. 


Despite its success in generating high-quality images, DPMs suffer from the drawbacks of prolonged inference time. 
Considerable interest has been expressed in minimizing the number of inference steps during the sampling process to speed up generation, while preserving the quality of generated images. Such works include generalizing DDPM~\citep{ddpm} to non-Markovian processes~\citep{song2021ddim}, deriving optimal variance during sampling~\citep{bao2022analyticdpm}, thresholding the pixel values as additional regularization~\citep{saharia2022photorealistic}, or developing pseudo numerical methods for solving differential equations on manifolds~\citep{liu2022pseudo}.


Though showing promising performance, 
% few of them has examined the connection between the training and sampling of DDPM, theoretically and empirically, to study the cause of the prediction errors.
none of them have theoretically and empirically examined the discrepancy between the training and sampling process of DPM. 
% In this paper, we focus on the error accumulation problem during sampling, which is less explored by previous works.
% % We commence by defining two types of error sources that occur during the sampling process: network prediction errors and the exposure bias problem.
% % We commence by identifying the network prediction errors that DDPM makes during sampling, and one of the major source, namely exposure bias problem, of such errors.
% We commence by pinpointing the network prediction errors produced by DDPM throughout the sampling process. We also shed light on one of the predominant origins of these errors, specifically the phenomenon known as the exposure bias problem.
% The training of DDPM involves optimizing the evidence lower bound.
% % This inherent requirement inevitably results in prediction errors during inference, attributable to the network's generalization capabilities.
% Moreover, a large number of diffusion steps of DDPM ensures that small step sizes are taken, which guarantee the Gaussian assumption holds~\citep{xiao2022diffusiongan}. Consequently, 
% a reduction in the number of time steps during the sampling phase can lead to larger prediction errors.
%We term these two types of errors as network prediction errors.
%
%Moreover, 
If we take a closer look at the training of DPM, at each time step $t$, ground truth samples $x_0$ are given to produce corrupted samples $x_t$ with noise $\epsilon_t$. The DPM takes both $x_t$ and $t$ as input to predict the noise $\epsilon_t$. During sampling, one is required to synthesize data samples from white noise without the knowledge of the ground truth distributions. Coupled with the prediction errors of the network,
this training-sampling discrepancy produces errors that could progressively accumulate during inference. This error arising from the difference between training and inference resembles the exposure bias problem as identified in autoregressive generative models~\citep{ICLR16seq, schmidt-2019-generalization}, given that the network is solely trained with the corrupted ground truth samples, rather than the network predicted samples.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{images/model.pdf}
     \caption{The comparison of \textit{TS}-DDPM (ours) and DDPM. The orange and blue arrows denote the time-state coupling at each denoising step of \textit{TS}-DDPM and DDPM, respectively. In \textit{TS}-DDPM, we search for coupled time step within the $[t-w/2, t+w/2]$ window, until the cutoff time step $t_c$.}
    \label{fig:model}
\end{figure}

% The orange cross highlights the cutoff value in TS-DDPM.

% The network prediction errors are inevitably avoided in the training of DDPM, thus the discrepancy between training and inference 
% which makes it difficult to be reduced via alternating sampling algorithms alone.
% which makes alternative sampling algorithms appealing.
In this work, we focus on the exposure bias problem during sampling. 
\citet{ning2023input} propose to add perturbation to training samples to alleviate the exposure bias problem, which is sub-optimal since the retraining of DPM is computationally expensive.
% , \textcolor{red}{making it difficult to scale to high-resolution images}.
Given that the time step $t$ is directly linked to the corruption level of the data samples, we theoretically and empirically show that by adjusting the next time step $t-1$ during sampling according to the variance of the current generated samples, one can effectively alleviate the exposure bias.
We search for such a time step within a window $t_w$ surrounding the current time step to restrict the denoising progress.
Furthermore, based on the error patterns that the network makes on the training samples, we propose the use of a cutoff time step $t_c$.
% where once reached, we do not adjust time step anymore.
For time steps larger than $t_c$, we search for the suitable time step within $t_w$. While for time steps smaller than $t_c$, we keep the original time step.
Intuitively, it also suits the nature of a DPM, since the corruption level is smaller for small time steps. 
We refer to our sampling method as Time-Shift Sampler. 
% Figure \ref{fig:model} presents a comparison of the \textcolor{red}{DDPM} variant of our method (\textit{TS}-DDPM) with the original DDPM. 
Figure~\ref{fig:model} presents the comparison between DDPM, the stochastic sampling method, and its time-shift variant \textit{TS}-DDPM. 
In summary, our contributions are:


\begin{itemize}
    \item We theoretically and empirically study the exposure bias problem of diffusion models, which is often neglected by previous works.
    \item We propose a new sampling method called Time-Shift Sampler to alleviate the exposure bias problem, which avoids retraining the models. Our method can be seamlessly integrated to existing sampling method by only introducing minimal computational cost.
    %for such aim 
    % \citep{ning2023input}.
    \item Our Time-Shift Sampler shows consistent and significant improvements over various sampling methods on commonly used image generation benchmarks, indicating the effectiveness of our framework. Notably, our method improves the FID score on CIFAR-10 from F-PNDM~\citep{liu2022pseudo} by 44.49\% to 3.88 with only 10 sampling steps.
\end{itemize}






==> sec2-relatedwork.tex <==
\section{Related Work}
\textbf{Denoising Diffusion Probabilistic Model.} The denoising diffusion probabilistic model (DDPM) was first introduced by \citet{ddpm_ori} and further advanced by \citet{improved_ddpm}, where they include variance learning in the model and optimize it with a new weighted variational bound. \citet{song2020score} further connect DDPMs with stochastic differential equations by considering DDPMs with infinitesimal timesteps. They also find that both score-based generative models~\citep{song2019generative} and that DDPMs can be formulated by stochastic differential equations with different discretization. Some variants of DDPMs are introduced recently, including the variational diffusion model (VDM)~\citet{kingma2021variational} that also learns the forward process, and consistency model~\citep{song2023consistency} and rectified flow model~\citep{liu2022flow}, both of which aim to learn to generate natural images in one inference step.

DDPMs are initially applied in the pixel space achieving impressive success in generating images of high quality, however, they suffer from the significant drawbacks such as prolonged inference time and substantial training cost. \citet{latent} propose to use a diffusion model in the latent image space, which drastically reduces the computational time and training cost. DDPMs have been widely used in different fields, for example controllable image generation~\citep{latent,choi2021ilvr,zhang2023adding,mou2023t2i}, language generation~\citep{zhang2023diffusum,ye2023dinoiser,lin2022genie}, image super-resolution~\citep{saharia2022image} and video generation~\citep{hu2023lamd,karras2023dreampose,he2022latent}.

\textbf{DDPM Accelerator.} Though diffusion models have shown powerful generation performance, it normally takes hundreds of steps to generate high-quality images~\citep{ddpm}. To accelerate the generation speed, \citet{song2021ddim} propose the denoising diffusion implicit model (DDIM) which derives ordinary differential equations %(ODEs) 
for the diffusion model showing the possibility of generating high-quality images in much less steps. \citet{liu2022pseudo} introduce numerical solvers to further reduce the number of generation steps. \citet{bao2022analyticdpm} find that the variance in the backward process can be analytically computed and improve the quality of the generated images. 
% In their another work~\citep{bao2022estimating}, they further remove the diagonal variance matrix assumption and boost the image generation performance. 
\citet{bao2022estimating} further remove the diagonal variance matrix assumption and boost the image generation performance. 
\citet{lu2022dpm-solver} leverage a high-order ordinary differential equations solver to reduce the generation steps of a diffusion model to 10, while maintaining the image quality. We follow this line of research and propose a method to better select time steps.

==> sec3-method.tex <==

\section{Investigating Exposure Bias in Diffusion Probabilistic Models}

In this section, we first 
% take DDPM~\citep{ddpm} as an example to 
give a brief introduction of the training and inference procedure for Diffusion Probabilistic Models (DPMs). 
Then we empirically study the exposure bias problem in DPM by diving deep into the training and inference processes.
% We provide observations that support our method as discussed in the next section (Sec.~\ref{sec:method}).


\subsection{Background: Diffusion Probabilistic Models}
% Denoising Diffusion Probabilistic Models (DDPMs) 
% As a class of DPMs, 
DPM 
encompasses a forward process which induces corruption in a data sample (e.g., an image) via Gaussian noise, and a corresponding inverse process aiming to revert this process in order to generate an image from standard Gaussian noise. Given a data distribution $q(x_0)$ and a forward noise schedule $\beta_t\in(0,1),t=1\cdots T$, the forward process is structured as a Markov process, 
which can be expressed as:
\begin{equation}
\label{forward_ddpm}
    q(x_{1\cdots T}|x_0) = \prod_{t=1}^{T}q(x_t|x_{t-1})
\end{equation}
with the transition kernel $q(x_t|x_{t-1})=\mathcal{N}(x_t|\sqrt{\alpha_t}x_{t-1},\beta_t\mathbf{I})$, where $\mathbf{I}$ denotes the identity matrix, $\alpha_t$ and $\beta_t$ are scalars and $\alpha_t=1-\beta_t$. 
% The forward process, consequently, generates a sequence of noisy states, denoted as $x_1, x_2,\dots, x_T$. With a sufficiently large $T$, we achieve $x_T\sim \mathcal{N}(\mathbf{0},\mathbf{I})$. 
%Notably, 
With the reparameterization trick, the noisy intermediate state $x_t$ can be computed by the equation below:
\begin{equation}
\label{q_sample}
    x_t=\sqrt{\overline{\alpha}_t}x_0+\sqrt{1-\overline{\alpha}_t}\epsilon_t
\end{equation}
where $\overline\alpha_t=\prod_{i=1}^{t}\alpha_t$ and $\epsilon_t\sim\mathcal{N}(\mathbf{0},\mathbf{I})$.
% \begin{equation}
% \label{eq2}
% \begin{split}
%     q(x_t|x_0) &=
%     \mathcal{N}(x_t|\sqrt{\overline{\alpha}_t}x_0,(1-\overline{\alpha}_t)\mathbf{I})
% \end{split}
% \end{equation}
% only depends on $x_0$ and parameter $\overline\alpha_t=\prod_{i=1}^{t}\alpha_t$, and $x_t$ can be computed by marginalizing intermediate steps along the sequence:
% \begin{equation}
% \label{eq2}
% \begin{split}
%     q(x_t|x_0) &=
%     \mathcal{N}(x_t|\sqrt{\overline{\alpha}_t}x_0,(1-\overline{\alpha}_t)\mathbf{I})
% \end{split}
% \end{equation}
%Moreover, 
% With the reparameterization trick, the sample $x_t$ at any step $t$ can be obtained as:
% \begin{equation}
% \label{q_sample}
%     x_t=\sqrt{\overline{\alpha}_t}x_0+\sqrt{1-\overline{\alpha}_t}\epsilon
% \end{equation}
% where $\overline\alpha_t=\prod_{i=1}^{t}\alpha_t$ and $\epsilon\sim\mathcal{N}(\mathbf{0},\mathbf{I})$.
According to the conditional Gaussian distribution, we have the transition kernel of backward process as:
\begin{equation}
    p(x_{t-1}|x_t,x_0) = \mathcal{N}(\Tilde{\mu}_t(x_t,x_0),\Tilde{\beta}_t)
\end{equation}
where $\Tilde{\beta}_t=\frac{1-\overline{\alpha}_{t-1}}{1-\overline{\alpha}_t}\beta_t$ and $\Tilde{\mu}_t=\frac{\sqrt{\overline{\alpha}_{t-1}}\beta_t}{1-\overline{\alpha}_t}x_0+\frac{\sqrt{\alpha_t}(1-\overline{\alpha}_{t-1})}{1-\overline{\alpha}_t}x_t$. Considering Equation~\ref{q_sample}, $\Tilde{\mu}_t$ can be further reformulated as $\Tilde{\mu}_t=\frac{1}{\sqrt{\alpha_t}}(x_t-\frac{1-\alpha_t}{\sqrt{1-\overline{\alpha}_t}}\epsilon_t)$. During training, a time-dependent neural network is optimized by either learning  $\Tilde{\mu}_t$ or $\epsilon_t$. Empirically, \citet{ddpm} observes that predicting $\epsilon_t$ works better. The learning target is to optimize the variational lower bound of the negative log-likelihood, which could also be interpreted as minimizing the KL divergence between the forward and backward process. In practice, \citet{ddpm} further simplifies the loss function as:
\begin{equation}
\label{loss_function}
    \mathcal{L}_{simple}= \mathbb{E}_{t,x_0,\epsilon_t\sim \mathcal{N}({\bf 0},\mathbf{I})}[\|\epsilon_{\theta}(x_t, t)-\epsilon_t \|_2^2] 
\end{equation}

% The transition kernel of backward process is assumed to follow below Gaussian distribution:
% \begin{equation}
%     p_{\theta}(x_{t-1}|x_t)=\mathcal{N}(x_{t-1};\mu_{\theta}(x_t,t),\Sigma_{\theta}(x_t,t))
% \end{equation}
% where $\mu_{\theta}(x_t,t)$ can be further parameterized as:
% \begin{equation}
%     \mu_{\theta}(x_t,t) =\frac{1}{\sqrt{\alpha_t}}(x_t-\frac{1-\alpha_t}{\sqrt{1-\overline{\alpha}_t}}\epsilon_{\theta}(x_t,t))
% \end{equation}
% In the work of~\citet{ddpm}, the variance $\Sigma_{\theta}(x_t,t)$ is set to a untrained time dependent constants $\sigma_t^2\mathbf{I}$, and $\sigma_t^2$ can either be $\beta_t$ or $\frac{1-\overline{\alpha}_{t-1}}{1-\overline{\alpha}_t}\beta_t$. 

% During the training phase, a time-dependent diffusion model is optimized by either learning  $\mu_{\theta}$ or $\epsilon_t$. Empirically, it has been found~\citep{ddpm} that the training works better by directly predicting $\epsilon_t$. The learning target is to optimize the variational lower bound of the negative log-likelihood, which could also be interpreted as minimizing the KL divergence between the forward and backward process. In practice, \citet{ddpm} further simplified the loss function as:


We present the training and sampling algorithms of the original Denoising Diffusion Probabilistic Models (DDPM)~\citep{ddpm} in Algorithm~\ref{algorithm-1} and \ref{algorithm-2}, respectively.


\vspace{-\intextsep}


\begin{minipage}[!htbp]{0.48\textwidth}
\begin{algorithm}[H]
    %\centering
    \caption{Training}\label{algorithm-1}
    \begin{algorithmic}[1]
    \Repeat
    \State $x_0\sim q(x_0)$
    \State $t \sim \text{Uniform}({1, \cdots, T})$ 
    \State $\epsilon \sim \mathcal{N}(\mathbf{0}, \textbf{I})$  Compute $x_t$ using Eq~\ref{q_sample}
    \State Take gradient descent step on %\\ $\nabla||\epsilon-\epsilon_{\theta}(x_t)||^2$
    \State $\nabla||\epsilon-\epsilon_{\theta}(x_t,t)||^2$
    \Until {converged}
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\hfill 
\begin{minipage}[!htbp]{0.48\textwidth}
\begin{algorithm}[H]
% \setstretch{1.2}
    %\centering
    \caption{Sampling}\label{algorithm-2}
    \begin{algorithmic}[1]
    \State $x_T \sim \mathcal{N}(0,\mathbf{I})$
        \For{$t = T,\cdots, 1$}
        \State  $z \sim \mathcal{N}(\mathbf{0},\mathbf{I})$ if $t > 1$, else $z=0$
        \State  $x_{t-1} = \frac{1}{\sqrt{\alpha_t}}(x_t-\frac{1-\alpha_t}{\sqrt{1-\overline\alpha_t}}\epsilon_{\theta}(x_t,t))+\sigma_tz$
        \EndFor \\ 
    \Return $x_0$
    \end{algorithmic}
\end{algorithm}
\end{minipage}


%  \citet{song2021ddim} propose a more general non-Markov process bearing the same marginal distribution of $x_t$ and index this process by $\sigma_t$: 
% \begin{equation}
% \label{ddim_process}
%  \begin{aligned} 
%     &q_{\sigma}(x_{1\cdots T}|x_0)=q_{\sigma}(x_T|x_0)\prod_{t=2}^{T}q_{\sigma}(x_{t-1}|x_t,x_0) \\ 
%     &q_{\sigma}(x_{t-1}|x_t,x_0) = \mathcal{N} (x_{t-1}| \Tilde{\mu}(x_t,x_0), 
%     \sigma_t^2)  \\
%     &\Tilde{\mu}(x_t,x_0) =\sqrt{\overline\alpha_{t-1}}x_0+(\sqrt{1-\overline{\alpha}_{t-1}-\sigma_t^2})\frac{x_t-\sqrt{\overline\alpha_t}x_0}{\sqrt{1-\overline\alpha_{t}}}
%  \end{aligned}
% \end{equation}
% The above equation encompasses two prevalent diffusion models, namely DDIM and DDPM when the $\sigma_t^2$ is respectively designated to zero and $\Tilde{\beta}_t =\frac{\overline\beta_{t-1}}{\overline\beta_t}\beta_t$, where $\overline{\beta}_t=1-\overline\alpha_t$. 
% % respectively.
% The backward process can be regarded as a denoising process, which progressively eliminates noise from the current step $x_t$ to obtain the previous state $x_{t-1}$, and finally reach $x_0$:
% \begin{equation}
% \label{backward_process}
% \begin{aligned}
%     &p(x_{0:T}) = p(x_T)\prod_{t=1}^Tp(x_{t-1}|x_t) \\
%     &p(x_{t-1}|x_t)=\mathcal{N}(x_{t-1}|\Tilde{\mu}_t(x_t,\frac{1}{\sqrt{\overline\alpha_t}}(x_t+\sqrt{1-\overline\alpha_t}\epsilon_t(x_t)))
% \end{aligned}
% \end{equation}


% During training phase, a time-dependent diffusion model is optimized by either learning  $\Tilde{\mu}_t$ or $\epsilon_t$. Empirically, it has been found~\citep{ddpm} that the training works better by directly predicting $\epsilon_t$. The learning target is to optimize the variational lower bound of the negative log-likelihood, which could also be interpreted as minimizing the KL divergence between the forward and backward process. In practice, \citet{ddpm} further simplified the loss function as:
% \begin{equation}
% \label{loss_function}
%     \mathcal{L}_{simple}= \mathbb{E}_{t,x_0,\epsilon\sim \mathcal{N}({\bf 0},\mathbf{I})}[\|\epsilon_{\theta}(\widetilde{x}, t)-\epsilon \|_2^2] 
% \end{equation}
% where $\widetilde{x}=\sqrt{\overline{\alpha}_t} x_0+\sqrt{1-\overline{\alpha}_t}\epsilon$. Upon the completion of the training of the diffusion model, we can sample a start state $x_T\sim \mathcal{N}(\mathbf{0},
% \mathbf{I})$ and adhere to the backward process to generate a data sample $x_0$. The training and inference processes are presented in Algorithm \ref{algorithm-1} and \ref{algorithm-2}~\citep{ddpm}, respectively.





\subsection{The Exposure Bias in Diffusion Probabilistic Models}
\label{sec:exposure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\columnwidth]{images/cifar10_error.png}
%     \caption{CIFAR-10 prediction errors of training samples for different number of sampling steps. (a): 10 steps; (b): 20 steps; (c): 50 steps; (d) 100 steps.}
%     \label{fig:cifar_error_by_step}
% \end{figure}


\begin{wrapfigure}[14]{r}{0.4\textwidth}
% \vspace{-10pt}
  \vspace{-\intextsep}
  \hspace*{-.75\columnsep}
  \begin{center}
  \includegraphics[width=0.4\columnwidth]{images/var_by_step_heat.pdf}
  \end{center}
  \vspace{-\intextsep}
  \caption{The density distribution of the variance of 5000 samples from CIFAR-10 by different time steps.}
  \label{fig:data_var_by_step}
\end{wrapfigure}


In this section,
% we provide empirical evidence of the exposure bias problem in Diffusion Models demonstrated with CIFAR-10. 
we empirically demonstrate 
the phenomenon related to
the exposure bias problem in DPM using CIFAR-10 dataset~\citep{krizhevsky2009learning}. 
We first present the variance distribution of the corrupted samples by different time steps in the forward process during training. Models exposed to a wider range of inputs during training tend to exhibit greater robustness to noise and are consequently less susceptible to exposure bias. 
To further study the behavior of the network during the backward sampling process, we also examine the evolution of prediction errors during sampling. We use DDIM~\citep{song2021ddim} sampler to conduct this experiment, as it gives a deterministic sampling process. 


Figure \ref{fig:data_var_by_step} presents the changes in variance of sample distributions for different time steps.
At each step, we estimate the corrupted image samples with the network predicted noise using Equation \ref{q_sample}.
We present the details of the figure in Appendix~\ref{appendix:fig_details}.
At time step 0, %where no noise is added, 
ground truth images serve as the current samples. The distribution of the variance of the ground truth samples spans an approximate range of $(0, 0.8)$, showing the diversity of the sample distributions.
As the noise is gradually added to the ground truth samples, the span of the variance becomes narrower and narrower.
Following 400 steps, the changes in the span range of the variance become stable, and gradually shift towards a narrow range surrounding the variance of white noise. 
%, which equals 1.0.
The evolution of the sample variance across different time steps indicates that the network exhibits a lower sensitivity to the early steps of the forward process of DPM, as the variance of the samples can be distributed more sparsely within a broader range. Conversely, the network can be more sensitive to the later steps (e.g., after 400 steps), as we progressively approach white noise. 
The constricted variance range during the later stages implies that minor prediction errors during sampling can significantly impact overall performance.



\begin{figure*}[htbp]
\label{cifar-error}
\centering
\subfloat[\scriptsize{10 steps}]{\includegraphics[width=0.24\textwidth]{images/cifar10_error_acc_10.png}
}
\hfil
\subfloat[\scriptsize{20 steps}]{\includegraphics[width=0.24\textwidth]{images/cifar10_error_acc_20.png}
}
\hfil
\subfloat[\scriptsize{50 steps}]{\includegraphics[width=0.24\textwidth]{images/cifar10_error_acc_50.png}
}
\hfil
\subfloat[\scriptsize{100 steps}]{\includegraphics[width=0.24\textwidth]{images/cifar10_error_acc_100.png}
}
\caption{CIFAR-10 prediction errors of training samples for different numbers of sampling steps.}
\label{fig:cifar_error_by_step}
\end{figure*}



In the second experiment, given a specific number of sampling steps, we compute the mean squared errors between the predicted samples and the ground truth samples at each step, 
% and present the results in Figure \ref{fig:cifar_error_by_step}.
as presented in Figure \ref{fig:cifar_error_by_step}. Details for plotting this figure are presented in Appendix~\ref{appendix:fig_details}. 
It can be seen that the evolution of prediction errors adheres to a consistent pattern: initially decreasing before incrementally accumulating as the sampling process progresses.
This phenomenon may be attributed to two possible factors: (1) The sampling process originates from white noise, which does not contain any information about the resultant sample distributions. In early stages, with fewer sampling steps, the error accumulation is less serious, thus the network gradually shapes the predicted distribution into the target distribution.
% a distribution that mirrors the ground truth sample distribution, 
% the distribution will be more similar to the sample distribution than the white noise.
% % Also the network is more robust to noisy inputs at this stage, since it exhibits a broader range of input variance as presented in Figure~\ref{fig:data_var_by_step}.
% Hence, in the early stages, the errors are reduced.
% as the white noise is shaped into a distribution that mirrors the ground truth sample distribution by DPM. 
% So for a short period of time, the errors decrease as the white noise is quickly molded into a distribution that mimic the ground truth sample distribution by Diffusion Models.
(2) In the later stages, the network is more robust to the noisy inputs as discussed above. However, due to the exposure bias, the network inevitably makes errors at each step and this errors accumulate along the sequence, resulting in a slow but steady progress in error accumulation and larger errors in the end. 

In conclusion, the above two experiments together show that during backward sampling process, the accumulated prediction error, which arises from the exposure bias and the capability of the network, could strongly impact the final results. 
% This demonstrates the importance and the potential of result improvements of alleviating exposure bias in diffusion models.
This demonstrates the importance of alleviating exposure bias in DPM, which could potentially lead to improved results.

% the exposure bias problem impacts the generated sample distributions. The network is still trying to predict distributions as authentic as possible; however, 
% % due to the discrepancy between training and inference, 
% due to the training-sampling discrepancy, 
% the network can only deduce such distributions from its own parameters and the generated sample distributions it obtained so far, without the guidance from the ground truth sample distributions,
% % That leads to the accumulated errors as shown in Figure \ref{fig:cifar_error_by_step}.
% which leads to accumulated errors in Figure \ref{fig:cifar_error_by_step}.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\columnwidth]{images/var_by_step_heat.png}
%     \caption{The density distribution of the variance of 5000 samples from CIFAR-10 by different time steps}
%     \label{fig:data_var_by_step}
% \end{figure}

% We also present the changes in variance of sample distributions for different time steps in Figure \ref{fig:data_var_by_step}. 




% \begin{algorithm}
% \caption{Time-asymmetric sampling with time intervals cutoff }\label{alg:sampling}
% \SetAlgoVlined
% \Input{Source condition $x$; number of steps M; model parameters $\theta$; cutoff value $t_c$ }
% \Output{Predicted target $\hat{y}$}

% \textbf{Initialize}:
% Time steps $\{t_i \}_{i=0}^{M}$ uniformly taken from [$t_c$, 1] ($t_c \gg 0$); $\hat{z}_{t0} \sim \mathcal{N}(0,1)$

% \For{ $i=1$ to $M$ }{
%     $\hat{z}_0 \leftarrow z_{\theta}(\hat{z}_{t_{i-1}}, x, t_c) $
    
%     $\hat{\epsilon} \leftarrow \frac{\hat{z}_{t_{i-1}} - \alpha(t_c) \hat{z}_0 }{\delta(t_c) } $

%     $\hat{z}_{t_i} \leftarrow \alpha(t_i) \hat{z}_0 + \delta(t_i) \hat{\epsilon} $
% }

% Output $\hat{z}_{t_M} $ as $\hat{y}$

% \end{algorithm}

\section{Alleviating Exposure Bias via Time Step Shifting}
\label{sec:method}

In the backward process of Diffusion Probabilistic Models (DPM), the transition kernel is assumed to adhere to a Gaussian distribution. To maintain this assumption, the difference between two successive steps must be sufficiently small, thereby necessitating the extensive training of DPM with hundreds of steps. 
% The noise schedule defines the level of noise present at a specific time step within the diffusion process, as depicted in Equation~\ref{q_sample}. 
As previously discussed, the network prediction error coupled with discrepancy between training and inference phases inevitably results in the problem of exposure bias in DPM. We introduce $\mathcal{C}(\Tilde{x}_t,t)$--referred to as the input couple for a trained DPM--to describe this discrepancy, which can be expressed as:
\begin{equation}
    \mathcal{C}(\Tilde{x}_t,t)=e^{-dis(\Tilde{x}_t,x_t)}
\end{equation}
where $\Tilde{x}_t$ and $x_t$ represent the network input and ground truth states at time step $t$, respectively, and $dis(\cdot,\cdot)$ denotes the Euclidean distance. Consequently, during the training phase, the relationship $\mathcal{C}(\Tilde{x}_t,t)=1$ holds true for all time steps, as the network always takes ground truth $x_t$ as input. Moreover, a better coupling expressed by $\mathcal{C}(\Tilde{x}_t,t_s)$ reduces the discrepancy between training and inference, thereby alleviating exposure bias. Previous works~\citep{zhang2023lookahead, ning2023input} have empirically and statistically affirmed that the network prediction error of DPM follows a normal distribution. In conjunction with Equation~\ref{q_sample}, during the backward process at time step $t$, the predicted next state denoted as $\hat{x}_{t-1}$ could be represented as:
\begin{equation}
\label{pred_x}
\begin{aligned}
    \hat{x}_{t-1} &= x_{t-1}+\phi_{t-1}e_{t-1} \\
    & = \sqrt{\overline\alpha_{t-1}}x_0 + \sqrt{1-\overline\alpha_{t-1}}\epsilon_{t-1} + \phi_{t-1}e_{t-1} \\
    &=\sqrt{\overline\alpha_{t-1}}x_0+\lambda_{t-1}\Tilde{\epsilon}_{t-1} 
\end{aligned}
\end{equation}
In this equation, $\lambda_{t-1}^2=\phi_{t-1}^2+(1-\overline{\alpha}_{t-1})$, $x_{t-1}$ denotes the ground truth at time step $t-1$, $\phi_{t-1}e_{t-1}$ represents the network prediction errors, and $e_{t-1}$, $\epsilon_{t-1}$ and $\Tilde{\epsilon}_{t-1}$ conform to a normal distribution. Upon observing that Equation~\ref{pred_x} and Equation~\ref{q_sample} share a similar structure which is the ground truth $x_0$ plus Gaussian noise with variable variance, we propose the subsequent assumption.
\newtheorem{assumption}{Assumption}[section]
 \begin{assumption}\label{asump1}
During inference at time step $t$, the next state $\hat{x}_{t-1}$ predicted by the network, may not optimally align with time step $t-1$ within the context of the pretrained diffusion model. In other words, there might be an alternate time step $t_s$, that potentially couples better with $\hat{x}_{t-1}$: 
\begin{equation}
 {\exists}s\in \{1\cdots T\}, \quad s.t. \quad \mathcal{C}(\hat{x}_{t-1}, t_s) \geq \mathcal{C}(\hat{x}_{t-1},t-1)
\end{equation}
\end{assumption}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.0\columnwidth]{images/celeba_10_win5.png}
%     \caption{celeba discrepancy}
%     \label{celeba_discrepancy_10_5}
% \end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.96\columnwidth]{images/cifar10_win_5_step_10_0_9.pdf}
    \caption{The training and inference discrepancy of DDIM with 10 sampling steps on CIFAR-10. The dashed line in each column denotes the couple of predicted $\hat{x}_{t}$ and $t$. Points on the right side of the dashed line mean that the corresponding time steps  couple better with $\hat{x}_{t}$ than time step $t$.}
    \label{cifar10_discrepancy_10_5}
\end{figure}
To verify our assumption, we initially conduct a statistical examination of the discrepancy between training and inference in a pretrained diffusion model. A sample size of $5000$ instances was randomly selected from the CIFAR-10 training set and Equation~\ref{q_sample} was utilized to generate ground truth states $x_t$ for a sequence of time steps. Subsequently, we compare the $\mathcal{C}(\hat{x}_{t},t)$ with $\mathcal{C}(\hat{x}_t,t_s)$. Details of plotting this figure are presented in Appendix~\ref{appendix:fig_details}. Here we show the results of $10$ inference steps in the backward process and only consider time step $t_s$ within the range of $t-6$ to $t+4$. As depicted in Figure~\ref{cifar10_discrepancy_10_5}, for certain backward steps, there are alternate time steps $t_s$ that display a stronger correlation with  the predicted next state $\hat{x}_{t}$ compared to time step $t$. We also observe that when approaching the zero time step, all nearby time steps converge to the same distribution. Similar findings were observed for other pretrained DPMs on different datasets including CelebA with varying settings, such as different numbers of inference steps and ranges of $t_s$. These results are further elaborated in Appendix~\ref{appendix:window}.


Our empirical findings lend substantial support to Assumption~\ref{asump1}. This naturally prompts the question: How can we identify the time step that best couples with the predicted $\hat{x}_{t-1}$? By optimizing the KL divergence between the predicted $\hat{x}_{t-1}$ and $x_s$ at time step $t_s$, we arrive at the following Theorem~\ref{thm1}, with the complete derivation provided in Appendix~\ref{appendix:derive}.


\newtheorem{thm}{\bf Theorem}[section]
\begin{thm}\label{thm1}
Given state $\hat{x}_t$ and assuming the predicted next state is $\hat{x}_{t-1}$, the optimal time step $t_s$ among those time steps closely surrounding $t-1$, which    best couples with $\hat{x}_{t-1}$, is determined to have the following variance:
\begin{equation}
   \begin{aligned}
    \sigma_{s} 
    % &\approx Tr(\hat{\Sigma}_{t-1})+ \frac{1}{d}||e||^2  
     % &\approx \sigma_{t-1} -(\frac{d-2}{d-1})||e||^2
     &\approx \sigma_{t-1} -\frac{||e||^2}{d \left( d-1 \right)}
    \end{aligned}
\end{equation}
where $d$ is the dimension of the input, $e$ represents the network prediction error, 
% $\hat{\Sigma}_{t-1}$ is the per-dimension covariance matrix of the predicted $\hat{x}_{t-1}$,
and $\sigma_{t-1}$ is the variance of the predicted $\hat{x}_{t-1}$. 
\end{thm}
The derivation of Theorem~\ref{thm1} mainly follows two steps: Firstly, we optimize the KL divergence between $x_s$ and $\hat{x}_{t-1}$ to obtain the variance of $x_s$; Secondly, we estabilish the relationship between the covariance matrix of the $\hat{x}_{t-1}$ distribution and the variance of the predicted $\hat{x}_{t-1}$. The results articulated in Theorem~\ref{thm1} could be further simplified to $\sigma_s \approx \sigma_{t-1}$, when $t$ is large and given the assumption that the network prediction error at the current time step is minimal. This assumption has been found to hold well in practice. 



\begin{wrapfigure}[22]{R}{0.5\textwidth}
    \vspace{-\intextsep}
  \hspace*{-.75\columnsep}
    \begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
    \centering
    \caption{Time-Shift Sampler}\label{algorithm-3}
    \begin{algorithmic}[1]
    \State \textbf{Input :} Trained diffusion model $\epsilon_{\theta}$; Window size $w$; Reverse Time series $\{T, T-1,\cdots, 0 \}$; Cutoff threshold $t_c$ %$\sigma_t=0$ for DDIM and $\sigma_t=\sqrt{\frac{1-\overline\alpha_{t-1}}{1-\overline\alpha_t}}\sqrt{1-\frac{\overline\alpha_t}{\overline\alpha_{t-1}}}$ for DDPM;
    \State \textbf{Initialize:} $x_T\sim \mathcal{N}(\mathbf{0},\mathbf{I})$ ; $t_s=-1$
    \For{$t = {T, T-1,.., 0}$}
    \State If $t_s \neq -1$ then  $t_{next} = t_s$ else $t_{next}=t$
    % \State $z\sim \mathcal{N}(\mathbf{0},\mathbf{I})$, if $t>1$ else $z=\mathbf{0}$
    \State $\epsilon_{t} = \epsilon_{\theta}(x_t,t_{next}))$
    \State take a sampling step with $t_{next}$ to get $x_{t-1}$
    \If{$t>t_c$}
    \State Get variance for time steps within the window: $\Sigma=\{1-\overline\alpha_{t-w/2},1-\overline\alpha_{t-w/2+1},\cdots,1-\overline\alpha_{t+w/2}\}$
    % \State $\hat{x}_{t-1}=\sqrt{\overline\alpha_{t-1}}(\hat{x}_0) + \sqrt{1-\overline\alpha_{t-1}-\sigma_t^2}\epsilon_{\theta}^{(t)}(x_t)+\sigma_t\epsilon_t$
    \State $t_s = \mathop{\arg\min}_{\tau} || var(x_{t-1}) - \sigma_{\tau}  ||$, for $\sigma_{\tau} \in \Sigma$ and $\tau \in [t-w/2, t+w/2]$
    % \State $\overline\alpha_{t-1}^s$ = compute\_alpha($\beta$, $t_s$)
    % \State $\hat{x}_{t-1}=\sqrt{\overline\alpha_{t-1}^s}(\hat{x}_0) + \sqrt{1-\overline\alpha_{t-1}^s-\sigma_t^2}\epsilon_{\theta}^{(t)}(x_t)+\sigma_t\epsilon_t$
    % \State $\hat{x}_0=\frac{x_t-\sqrt{1-\alpha_t}\epsilon^{(t)}_{\theta}(x_t)}{\sqrt{\alpha_t}}$
    % \State $t = \mathop{\arg\min}_{t'}\Tilde{\sigma}(\hat{x}_{t-1})$
    \Else
    \State $t_s=-1$
    \EndIf
    \EndFor \\ 
    \Return $x_0$
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\end{wrapfigure}


Based on the findings of Theorem~\ref{thm1}, we propose the Time-Shift Sampler, a method that can be seamlessly incorporated into existing sampling algorithms, such as Denoising Diffusion Implicit Models (DDIM)~\citep{song2021ddim}, Denoising Diffusion Probabilistic Models (DDPM)~\citep{ddpm} or sampling methods based on high-order numerical solvers~\citep{liu2022pseudo}. 
Moreover, in light of the earlier discussion that the model's predictions of nearby time steps tend to converge to the same distribution during the later stage of the inference process and the condition of large $t$ in the derivation in Appendix~\ref{appendix:derive}, we remove the time-shift operation when the time step is smaller then a predefined cutoff time step\footnote{We discuss the influence of the window size and the cutoff value in Sec.~\ref{sec:hyperparameter}.}.
Our algorithm is detailed in Algorithm~\ref{algorithm-3}. 
Specifically, given a trained DPM $\epsilon_{\theta}$, we sample for $x_t, t=1,2, \ldots, T$ using arbitrarily any sampling method.
For each time step $t>t_c$, where $t_c$ is the cutoff threshold, we replace the next time step $t_{next}$ with the time step $t_s$ that best couples with the variance of $x_{t-1}$ within a window of size $w$. 
In the search of such $t_s$, we first take a sampling step with the current $t_{next}$ to get $x_{t-1}$, which is used to compute the variance of $x_{t-1}$ as $var(x_{t-1})$. Then we get the variance $\Sigma$ of the time steps within the window. The optimal $t_s$ can be obtained via $\arg \min_{\tau}|| var(x_{t-1}), \sigma_{\tau}||$, for $\sigma_{\tau} \in \Sigma$. Finally, the obtained $t_s$ is passed to the next sampling iteration as $t_{next}$. We repeat this process until $t<t_c$, after which we perform the conventional sampling steps from the sampling method of choice.


% \begin{algorithm}[H]
% \caption{TS-DDIM/DDPM }\label{algorithm-3}
% \begin{algorithmic}
% \begin{minted}[mathescape, linenos]{python}
%  def ts-sampler(w, ):
     
% \end{minted}
% \end{algorithmic}
% \end{algorithm}






==> sec4-experiment.tex <==
\section{Experimental Setup}
% Experiment details including checkpoints used for  all datasets, diferent time series selection of ddim, dataset included in the experiment. Selection of window size , cutoff threshold.

% We refer to our method as TS-DDIM/DDPM.
We integrate our Time-Shift Samplers to various sampling methods including \textbf{DDPM}~\citep{ddpm}: the stochastic sampling method; 
\textbf{DDIM}~\citep{song2021ddim}: the deterministic version of DDPM;
\textbf{S-PNDM}~\citep{liu2022pseudo}: the sampling method based on second-order ODE solver; and
\textbf{F-PNDM}~\citep{liu2022pseudo}: the sampling method based on fourth-order ODE solver.
We term our Time-Shift Sampler as \textbf{\textit{TS}-\{$\cdot$\}} with respect to the baseline sampling methods. For example, the time shift variant of DDIM is referred to as \textit{TS}-DDIM.
% We compare our \textit{TS}-DDIM/DDPM to the original DDIM~\citep{song2021ddim} and DDPM~\citep{ddpm}, with $\sigma^2 = \Tilde{\beta}_n$ and $\sigma^2 = 0$ respectively.
% We also conduct experiments on sampling methods S-PNDM and F-PNDM~\citep{liu2022pseudo}, which are based on high-order numerical solvers, and their Time-Shift variant \textit{TS}-S-PNDM, \textit{TS}-F-PNDM.
Following DDIM, we consider two types of time step selection procedures during sampling, namely \textit{uniform} and \textit{quadratic}. 
% The details are presented in Appendix \ref{appendix:experiments}.
For $t_i < T$:
\begin{itemize}
    \item \textit{uniform}: we select time steps such that $t_i = \lfloor ci \rfloor$, for a constant value $c$
    \item \textit{quadratic}: we select time steps such that $t_i = \lfloor ci^2 \rfloor$, for a constant value $c$
\end{itemize}


We report main results using pre-trained DDPM on CIFAR-10~\citep{krizhevsky2009learning} and CelebA 64$\times$64~\citep{Liu_2015_ICCV}.
Moreover, based on DDIM sampler, a comparison to ADM-IP~\citep{ning2023input} is made, which uses ADM~\citep{NEURIPS2021_beatsgan} as the backbone model.
More experiments can be found in the appendix.
% and ImageNet 64$\times$64~\citep{cvpr09_imagenet}. 
% We adopt the pre-trained models trained with linear schedule (LS)~\citep{ddpm}. 
% The detailed information of the checkpoint used in our work is provided in Appendix \ref{appendix:experiments}.
We conduct experiments for varying sampling time steps, namely 5, 10, 20, 50, and 100. 
We use the Frechet Inception Distance (FID)~\citep{NIPS2017_FID} for evaluating the quality of the generated images.
% The detailed experimental setups are provided in Appendix \ref{appendix:experiments}.
We further discuss the influence of window sizes and cutoff values in Sec.~\ref{sec:hyperparameter}.
More details can be found in Appendix \ref{appendix:experiments}.


% The window size is selected according to the step sizes. For fewer sampling steps, a larger window size is preferred. 
% % An ablation study on window size selection is presented in Sec.\ref{sec:window}.
% The cutoff value is selected according to the variance distribution of training samples as depicted in Figure \ref{fig:data_var_by_step}. Specifically, we select the cutoff value within the range of $[200,400]$ for the model is more sensitive to larger time steps, and more tolerant to noise for smaller time steps. The selection of cutoff value is also dependent to the number of sampling steps we take, as some cutoff values are equivalent to specific settings 
% % (e.g. 200 and 250 are equivalent to models sampling with 10 steps using \textit{uniform} time step selection). 
% (e.g. 200 and 250 are equivalent to 10 sampling steps with \textit{uniform} time step selection).
% % We further discuss it in Sec. \ref{sec:cutoff}. 
% We further discuss the influence of hyperparameters in Sec.~\ref{sec:hyperparameter}.







==> sec5-results.tex <==
\section{Results}
\subsection{Main Results}


\begin{table}[!htbp]
    \centering
    \resizebox{\textwidth}{!}{%
    % \begin{tabular}{clccccc}
    \begin{tabular}{cllllll}
    % \hline
    \toprule
        Dataset & Sampling Method & 5 steps & 10 steps & 20 steps & 50 steps & 100 steps \\
    \hline
    % CIFAR10(LS) \\ 
    % \hline 
    \multirow{10}{*}{CIFAR-10} & DDIM (\textit{quadratic}) & 41.57 & 13.70 & 6.91 & 4.71 & 4.23 \\
     & \textit{TS}-DDIM(\textit{quadratic}) & \textbf{38.09 (+8.37\%)} & \textbf{11.93 (+12.92\%)} & \textbf{6.12 (+11.43\%)} & \textbf{4.16 (+11.68\%)} & \textbf{3.81 (+9.93\%)} \\
     % \hline
     \cline{2-7}
    & DDIM(\textit{uniform}) & 44.60 & 18.71 & 11.05 & 7.09 & 5.66 \\
    & \textit{TS}-DDIM(\textit{uniform}) & \textbf{35.13 (+21.23\%)} & \textbf{12.21 (+34.74\%)} & \textbf{8.03 (+27.33\%)}  & \textbf{5.56 (+21.58\%)} & \textbf{4.56 (+19.43\%)} \\
    % \hline
    \cline{2-7}
    & DDPM (\textit{uniform}) & 83.90 & 42.04 & 24.60 & 14.76 & 10.66 \\ 
    & \textit{TS}-DDPM (\textit{uniform}) & \textbf{67.06 (+20.07\%)} & \textbf{33.36 (+20.65\%)} & \textbf{22.21 (+9.72\%)} & \textbf{13.64 (+7.59\%)} & \textbf{9.69 (+9.10\%)} \\ 
    \cline{2-7}
    & S-PNDM (\textit{uniform}) & 22.53 & 9.49 & 5.37 & 3.74 & 3.71 \\ 
    & \textit{TS}-S-PNDM (\textit{uniform}) & \textbf{18.81(+16.40\%)} & \textbf{5.14 (+45.84\%)}	& \textbf{4.42 (+17.69\%)} & \textbf{3.71 (+0.80\%)} & \textbf{3.60 (+2.96\%)} \\ 
    \cline{2-7}
    & F-PNDM (\textit{uniform}) & 31.30 & 6.99 & 4.34 & 3.71 & 4.03 \\ 
    & \textit{TS}-F-PNDM (\textit{uniform}) & \textbf{31.11 (+4.07\%)} & \textbf{3.88 (+44.49\%)} & \textbf{3.60 (+17.05\%)} & \textbf{3.56 (+4.04\%)} & \textbf{3.86 (+4.22\%)} \\ 
    \hline 
    
    % CelebA 64x64 \\
    % \hline 
    \multirow{10}{*}{CelebA} & DDIM (\textit{quadratic}) & 27.28 & 10.93 & 6.54 & 5.20 & 4.96 \\
    & \textit{TS}-DDIM (\textit{quadratic}) & \textbf{24.24 (+11.14\%)} & \textbf{9.36 (+14.36\%)} & \textbf{5.08 (+22.32\%)} & \textbf{4.20 (+19.23\%)} & \textbf{4.18 (+15.73\%)} \\
    % \hline 
    \cline{2-7}
    & DDIM (\textit{uniform}) & 24.69 & 17.18 & 13.56 & 9.12 & 6.60 \\ 
    & \textit{TS}-DDIM (\textit{uniform}) & \textbf{21.32 (+13.65\%)} & \textbf{10.61 (+38.24\%)} & \textbf{7.01 (+48.30\%)} & \textbf{5.29 (+42.00\%)} & \textbf{6.50 (+1.52\%)} \\
    % \hline 
    \cline{2-7}
    & DDPM (\textit{uniform}) & 42.83 & 34.12 & 26.02 & 18.49 & 13.90 \\ 
    & \textit{TS}-DDPM (\textit{uniform}) & \textbf{33.87 (+20.92\%)} & \textbf{27.17 (+20.37\%)} & \textbf{20.42 (+21.52\%)} & \textbf{13.54 (+26.77\%)} & \textbf{12.83 (+7.70\%)} \\ 
    \cline{2-7}
    & S-PNDM (\textit{uniform}) & 38.67 & 11.36 & 7.51 & 5.24 & 4.74 \\ 
    & \textit{TS}-S-PNDM (\textit{uniform}) & \textbf{29.77 (+23.02\%)} & \textbf{10.50 (+7.57\%)} & \textbf{7.34 (+2.26\%)} & \textbf{5.03 (+4.01\%)} & \textbf{4.40 (+7.17\%)} \\ 
    \cline{2-7}
    & F-PNDM (\textit{uniform}) & 94.94 & 9.23 & 5.91 & 4.61 & 4.62\\ 
    & \textit{TS}-F-PNDM (\textit{uniform}) & \textbf{94.26 (+0.72\%)} & \textbf{6.96 (+24.59\%)} & \textbf{5.84 (+1.18\%)} & \textbf{4.50 (+2.39\%)} & \textbf{4.42 (+4.33\%)} \\ 
    % \hline 
    % ImageNet 64x64  \\ 
    % \hline 
    % \multirow{4}{*}{ImageNet} 
    % % & DDIM (\textit{quadratic}) & 171.11& 180.15 & 184.86 & 190.2&- \\
    % % & TS-DDIM (\textit{quadratic}) & - & - & -& -& - \\
    % % % \hline 
    % % \cline{2-7}
    % & DDIM (\textit{uniform}) & 146.19 & 42.51 & 25.60 & \textbf{20.17} & 18.76 \\ 
    % & TS-DDIM (\textit{uniform}) & \textbf{140.89 (+3.63\%)} & \textbf{41.68 (+1.95\%)} & \textbf{25.32 (+1.09\%)} & 20.26 (-0.45\%) & \textbf{17.20 (+8.32\%)} \\
    % % \hline 
    % \cline{2-7}
    % & DDPM (\textit{uniform}) & 96.99 & 62.90 & 35.72 & 21.47 & 18.27 \\ 
    % & TS-DDPM (\textit{uniform}) & \textbf{95.76 (+1.27\%)} & \textbf{61.78 (+1.78\%)}  & \textbf{34.83 (+2.49\%)} & 
    % \textbf{20.35 (+5.22\%)}& \textbf{17.70 (+3.12\%)} \\ 
    \bottomrule
    \end{tabular}
    }
    
    \caption{Quality of the image generation measured with FID $\downarrow$ on CIFAR-10 (32$\times$32) and CelebA (64$\times$64) with varying time steps for different sampling algorithms.}
    \label{tab:main}
\end{table}

In Table~\ref{tab:main}, we compare four sampling methods, namely DDIM, DDPM, S-PNDM and F-PNDM, and their Time-Shift variants on two datasets, where we vary the time steps and the time step selection procedures. 
We take larger window sizes for fewer sampling steps.
The cutoff value is within the range of $[200,400]$, and is dependent to the number of time steps we take. 
As expected, our Timer-Shift Sampler consistently improves the quality of the generated images with respect to that of the baseline sampling methods.
We observe that for time steps less than 20 with \textit{uniform} time step selection, the performance improvements are extremely significant as compared to the original sampling methods. 
To our surprise, even for very strong high-order sampling methods, our Time-Shift Sampler can still bring significant improvements. Notably, we obtain FID=3.88 with \textit{TS}-F-PNDM on CIFAR-10 using 10 sampling steps, which is better than DDIM on CIFAR-10 for 100 sampling steps.
% (e.g. more than 50\% gain in FID score).
% With \textit{uniform} time selection, large time steps are taken uniformly, which results in more time steps to be shifted before cutoff value as compared to \textit{quadratic} time selection. 
% We implement time shifts only for time steps exceeding the cutoff value. 
Our method also manages to improve the performance of the baseline sampling methods for both \textit{uniform} and \textit{quadratic} time selection, showing the versatility of our method.



% However, our algorithm shows less enhancement on the ImageNet dataset compared to others.
% This could potentially be attributed to the unique training setting of the DDPM model on ImageNet, which uses $4000$ time steps instead of $1000$ used for the other datasets.
% Models trained with larger time steps experience a more extensive range of noisy inputs. Consequently, this could results in a model that is more robust to noisy inputs during inference.



\subsection{Discussion on Efficiency and Performance}

\begin{wrapfigure}[20]{r}{0.6\textwidth}
    \centering
    \vspace{-\intextsep}
    \hspace*{-.75\columnsep}\includegraphics[width=\linewidth]{images/fid_curve_by_time.pdf}
    \caption{Sampling time VS FID on CIFAR-10 using DDPM as backbone with various sampling methods. We report the results of \{5,10,20,50\} sampling steps from left to right for each sampler, denoted with "$\times$" symbol. }
    \label{fig:cifar_time}
\end{wrapfigure}
Our Time-Shift Sampler involves searching for suitable time steps using computed variance of the generated samples, which inevitably brings additional computation during sampling.
To compare the efficiency of different sampling methods, we present the average sampling time\footnote{Test conducted on an AMD EPYC7502 CPU and a RTX 3090 GPU using Pytorch time estimation API.} in Figure~\ref{fig:cifar_time} by running each sampling method 300 times on CIFAR-10 using DDPM as backbone model. 
For all three sampling methods, the additional computation time during sampling with 5,10 and 20 sampling steps is negligible.  
The additional computation time is visually larger for 50 sampling steps. Yet, the actual additional computation time remains acceptable for a small backbone like DDPM.
For example, \textit{TS}-S-PNDM requires 9.71\% more sampling time on average than S-PNDM for 5,10 and 20 steps. For 50 steps, \textit{TS}-S-PNDM requires 9.86\% more sampling time than S-PNDM.
We report the detailed sampling time in Appendix~\ref{appendix:time}.
The additional computation time is also dependant to the choice of the backbone, which we further elaborate in Sec.~\ref{sec:adm_ip}.

% \begin{figure}[!htb]
%     \centering
%     \subfloat[]{\includegraphics[width=0.5\textwidth]{images/fid_curve_by_time.pdf}}
%      \centering
%     \subfloat[]{\includegraphics[width=0.5\textwidth]{images/fid_curve_adm_time.pdf}}
%     \caption{Sampling time VS FID on CIFAR-10 using DDPM (a) and ADM (b) as backbone with various sampling methods. We report the results of \{5,10,20,50\} sampling steps from left to right for each sampler, denoted with "$\times$" symbol.}
%     \label{fig:cifar_time}
% \end{figure}







\subsection{Comparison with Training-Required Method ADM-IP}
\label{sec:adm_ip}

\begin{table}[!htbp]
    \centering
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{lllllll}
      \hline
       Model & Sampling Method& 5 steps & 10 steps & 20 steps & 50 steps \\
      \hline
      ADM & DDIM & 28.98 & 12.11 & 7.14 & 4.45 \\
      ADM-IP & DDIM & 50.58 (-74.53\%) & 20.95 (-73.00\%) & 7.01 (+1.82\%) & \textbf{2.86 (+35.73\%)} \\
      ADM & \textit{TS}-DDIM & \textbf{26.94 (+7.04\%)} & \textbf{10.73 (+11.40\%)} & \textbf{5.35 (+25.07\%)} & 3.52 (+20.90\%) \\
      \hline
    \end{tabular}
    }
    \caption{Performance comparison on CIFAR-10 with ADM and ADM-IP as the backbone models. }
    \label{tab:adm_results}
\end{table}




\begin{wrapfigure}[17]{r}{0.5\textwidth}
  % \vspace{-\intextsep}
  % \hspace*{-.75\columnsep}
  
  % \begin{minipage}{\linewidth}
  %   \centering
  %   \resizebox{\textwidth}{!}{%
  %   \begin{tabular}{lllll}
  %     \hline
  %      & 5 steps & 10 steps & 20 steps & 50 steps \\
  %     \hline
  %     DDIM$\dag$ & 28.98 & 12.11 & 7.14 & 4.45 \\
  %     DDIM$\ddag$ & 50.58 (-74.53\%) & 20.95 (-73.00\%) & 7.01 (+1.82\%) & \textbf{2.86 (+35.73\%)} \\
  %     \textit{TS}-DDIM$\dag$ & \textbf{26.94 (+7.04\%)} & \textbf{10.73 (+11.40\%)} & \textbf{5.35 (+25.07\%)} & 3.52 (+20.90\%) \\
  %     \hline
  %   \end{tabular}
  %   }
  %   \vspace{-8pt}
  %   \captionof{table}{Performance comparison on CIFAR-10 with ADM($\dag$) and ADM-IP($\ddag$) as the backbone models. }
  %   \label{tab:adm_results}
    
  % \end{minipage}
  % \vspace{1em} % Adjust the vertical spacing between the figure and the table as needed
  % \begin{minipage}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/fid_curve_adm_time.pdf}
    % \vspace{-5pt}
    \vspace{-\intextsep}
    \caption{Sampling time VS FID on CIFAR-10 with ADM as backbone using DDIM and \textit{TS}-DDIM for sampling.}
    \label{fig:adm_time}
  % \end{minipage}
\end{wrapfigure}

Our method is also proven to be effective on alternative model architectures than DDPM. 
In this section we present the results on ADM~\citep{NEURIPS2021_beatsgan}, and the variant of ADM named ADM-IP~\citep{ning2023input}, which tries to alleviate exposure bias in DPM by retraining ADM with added input perturbation.
% As an alternative method to alleviate exposure bias in diffusion models, ADM-IP~\cite{ning2023input} retrains the ADM~\cite{NEURIPS2021_beatsgan} model with added input perturbation. 
We conduct our Time-Shift Sampler using ADM as backbone model to show the merits of our method as compared to ADM-IP.
We present the comparison on FID scores in Table~\ref{tab:adm_results} and the comparison on sampling time in Figure~\ref{fig:adm_time}.
The results indicate that when employing a small sampling step, which is favored in practice, ADM-IP performs much worse than the original ADM. As the number of sampling steps increases, the performance of ADM-IP improves. We manage to improve the performance of the ADM model with our method by a large margin. Note that we achieve these significant improvements without retraining the model as is required by ADM-IP.
We also obtain roughly the same sampling time for DDIM and \textit{TS}-DDIM with ADM as the backbone model. It makes our method more favorable in practice given merely zero additional cost for computation and significant performance improvements.



\subsection{Influence of Window Sizes and Cutoff Values}
\label{sec:hyperparameter}


% \begin{wrapfigure}[18]{r}{0.415\textwidth}
%   \begin{center}
%   \includegraphics[width=0.415\columnwidth]{images/window_compare4.png}
%   \end{center}
%   \caption{The impact of different window sizes on the quality of generated CIFAR-10 images with \textit{uniform} time step selection with cutoff value=300. }
%   \label{fig:window}
% \end{wrapfigure}

% \begin{wrapfigure}[20]{r}{0.45\textwidth}
%   \begin{center}
%   \includegraphics[width=0.45\columnwidth]{images/cutoff_compare_bar.png}
%   \end{center}
%   \caption{The impact of different cutoff values on the quality of generated CIFAR-10 images with \textit{uniform} time step selection. We adopt window size= \{40;30;8;2\} for \{10;20;50;100\} steps }
%   \label{fig:cutoff}
% \end{wrapfigure}


% \begin{figure}[!htbp]
% \centering
% \begin{minipage}{0.88\textwidth}
%     \centering
%     \begin{minipage}{0.51\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{images/window_compare4_bar.pdf}
%     \vspace{-\intextsep}
%     % \hspace*{-.75\columnsep}
%     \caption{FID of generated CIFAR-10 images using \textit{TS}-DDIM (\textit{uniform}) with cutoff value=300 using various window sizes. }
%     \label{fig:window}
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\textwidth}
%     \includegraphics[width=\textwidth]{images/cutoff_compare_bar_group.pdf}
%     \vspace{-\intextsep}
%     % \hspace*{-.75\columnsep}
%     \caption{FID of generated CIFAR-10 images using \textit{TS}-DDIM (\textit{uniform}) with various cutoff values. We adopt window size= \{40;30;8;2\} for \{10;20;50;100\} steps }
%     \label{fig:cutoff}
% \end{minipage}
% \end{minipage}
% \end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{images/hyperparameter_plot.pdf}
    \vspace{-\intextsep}
    % \hspace*{-.75\columnsep}
    \caption{FID of generated CIFAR-10 images using \textit{TS}-DDIM (\textit{uniform}) with (a) various window sizes using cutoff value=300; (b) various cutoff values using window size= \{40;30;8;2\} for \{10;20;50;100\} steps.}
    \label{fig:hyperparameter}
\end{figure}


% Our Time-Shift Sampler contains two hyperparamters, namely cutoff value and window size. We study the effect of these two hyperparameters on generation quality, and provide guidance for selecting the values in practice.



We first conduct a study on the effect of window sizes. The results are presented in Figure \ref{fig:hyperparameter} (a), where we fix the cutoff value=300, and vary the window sizes for different numbers of sampling steps. 
In the assessment of 10 and 20 sampling steps, larger window sizes 
% (up to 60 for sampling with 10 steps) 
are evaluated to ensure an adequate search space for a suitable time step.
% Contrastingly, in the context of 50 and 100 sampling steps, a comparative analysis is undertaken involving smaller window sizes, given the limitation of step size to be under 20 and 10 respectively.
And we adopt smaller window sizes for more sampling steps, given the limitation of step sizes. Figure~\ref{fig:hyperparameter} (a) illustrates that the Time-Shift algorithm is not sensitive to the selection of window size when using $10,20$ and $50$ sampling steps. While when the number of sampling step is increased, such as $100$ steps, the algorithm become more sensitive to the window size, which could be attributed to the enhanced accuracy of per-step predictions achievable with smaller step sizes.


% We observe that without overlapped time steps (i.e., when window size is smaller than step size), larger window size does not consistently yield optimal results
% (e.g. window size=50 underperforms 40 for 20 sampling steps).
% % To illustrate, when considering 20 sampling steps, using a window size of 50 underperforms in comparison to employing a window size of 40. 
% Such observation might be attributed to the less accurate estimations of time shifts, as larger step violates the assumption 

% precipitated by the network's inaccurate predictions in scenarios involving larger step size.

% However, when the number of sampling steps is increased, such as in a configuration of 100 steps, it is recommended to opt for a smaller window size, due to the enhanced accuracy of per-step predictions achievable with smaller step sizes.


% In summary, it can be deduced that larger window sizes are more effective for fewer sampling steps, whereas smaller window sizes tend to perform better when the number of sampling steps is increased.



% For 10 and 20 sampling steps, larger window sizes (up to 60 for 10 steps) are ablated to make sure we have enough search space for a suitable time step. 
% While for 50 and 100 sampling steps, we compare smaller window sizes, since step size is restricted to less than 20 and 10, respectively.
% We observe that for fewer sampling steps, without time steps overlapping (i.e. window size < step size), the maximum window size is not always optimal.
% For example, the maximum window size for 20 sampling steps is 50, which gives us worse performance than the model sampling with window size=40.
% It is possibly due to the inaccurate predictions the network makes for fewer sampling steps, which results in less accurate time shift estimation.
% If more sampling steps are taken (e.g. 100 steps), it is advised to take small window size, for the predictions per step are accurate enough with small step sizes.
% In general, we can conclude that sufficiently large window sizes work better for fewer sampling steps; while small window sizes work better for larger sampling steps.


% \subsection{Influence of the Cutoff Value}
% \label{sec:cutoff}

%To study the effect of cutoff values, we conduct ablation on the impact of different cutoff values on the image generation performance.
The influence of different cutoff values on the image generation performance on CIFAR-10 are presented in Figure~\ref{fig:hyperparameter} (b).
% (a similar study on other datasets can be found in Appendix \ref{appendix:cutoff}).
% The goal of the cutoff value is to restrict the Time-Shift Sampler to focus more on the time steps that the model is more sensitive to the noise, while maintaining the original time scheduling for the counterpart.
% \begin{wrapfigure}[20]{r}{0.45\textwidth}
%   \begin{center}
%   \includegraphics[width=0.45\columnwidth]{images/cutoff_compare_bar.png}
%   \end{center}
%   \caption{The impact of different cutoff values on the quality of generated CIFAR-10 images with \textit{uniform} time step selection. We adopt window size= \{40;30;8;2\} for \{10;20;50;100\} steps }
%   \label{fig:cutoff}
% \end{wrapfigure}
From the density distribution plot of the sample variance as discussed in Sec.~\ref{sec:exposure}, we can have a good estimation of the range of the cutoff values to be within $[200,400]$. %where the model is not as sensitive to noises as the larger steps.
While sampling with 10 steps, a smaller cutoff value (200) is preferred as compared to the scenarios with more sampling steps. 
One possible reason is that fewer sampling steps lead to larger step size, which makes more time-shift operations beneficial.

% As shown in Figure \ref{fig:hyperparameter} (b), the best FID is reached with cutoff value=200 for 10 sampling steps, while for the other sampling steps the best FID is reached with cutoff value=300. One possible reason for the different pattern with 10 sampling step is that the step size is much larger (100 vs. $<50$), which makes additional time-shift operations beneficial.
% For 20, 50 and 100 sampling steps, though we observe a similar pattern in changes of FID, the effect of the cutoff value is more drastic for fewer sampling steps. 
% Based on the observations, we can conclude that cutoff values are more effective when dealing with fewer sampling steps where the model takes larger step sizes to make predictions.
% And generally cutoff value=300 works best for sufficiently enough (e.g. $>10$) time steps.






%We also empirically study the effect of varying window sizes and cutoff values. 
% The optimal window size and cutoff values are empirically selected which yield improved performance. 
%We will further discuss these two hyper-parameters in Sec. \ref{sec:limitation}.






==> sec6-conclusion.tex <==
\section{Conclusion} 
% \subsection{Limitation and Future Work.}
% \label{sec:limitation}
% In this work, we introduce the Time-Shift Sampler, a training-free mechanism devised to mitigate the exposure bias problem inherent to the diffusion model, thereby enhancing the quality of generated images. Despite its efficacy, our sampler suffers from the limitation that it introduces two parameters, i.e.,   window size and cutoff value. We estimated their values based on the statistical analysis of training data. However, more advanced methods to % these empirical estimation is suboptimal. Since both cutoff value and window size are related to the noisy level of each step, it might be possible to 
% analytically derive the optimal value of these two parameters might be possible since both the cutoff value and the window size are related to the noise level of each step. We leave this further exploration to future work. We also foresee possibilities to use the concept of the Time-Shift Sampler in other Markovian processes where a reduction in processing steps is desired.

% \subsection{Conclusion}


In this paper, we have proposed a novel method to alleviate 
%we undertake a statistical and theoretical examination of the issue of 
% error accumulation, caused by 
the exposure bias problem in diffusion probabilistic models. Different from previous work, which tries to reduce exposure bias by retraining the diffusion model with extra noisy inputs, we demonstrate that this bias can be mitigated by identifying the timestep that most aligns with the subsequent predicted step. Furthermore, we theoretically derive the variance of this optimal next timestep. Leveraging these insights, we introduce a novel and training-free inference algorithm, the Time-Shifted Sampler, to alleviate exposure bias in diffusion models. Our algorithm can be seamlessly incorporated into existing 
% diffusion sampling 
sampling
algorithms for diffusion models including DDPM, DDIM, S-PNDM and F-PNDM. Extensive experimental results prove the effectiveness of our method.


